Quantum state transfer and time-dependent disorder in Quantum Chains

One of the most basic tasks required for Quantum Information Technology is the ability to connect different components of a Quantum Computer by quantum wires that obey the superposition principle. Since superpositions can be very sensitive to noise this turns out to be already quite difficult. Recently, it was suggested to use chains of permanently coupled spin-1/2 particles (quantum chains) for this purpose. They have the advantage that no external control along the wire is required during the transport of information, which makes it possible to isolate the wire from sources of noise. We first give an introduction to basic quantum state transfer and review existing advanced schemes by other authors. We then show a new result that demonstrates the stability of the scheme [1] against disorder that is approximately constant during one application of the channel, but time-dependent with respect to multiple applications.

==> di <==
< such as Josephson junctions with charge qubits~\cite{Bruder2005a,Romito2,Tsomokos2006},
---
> such as Josephson junctions with charge qubits~\cite{Bruder2005a,Tsomokos2006},
141c141
< Hamiltonians can at least be \emph{simulated} are NMR qubits~\cite{Suter2006,Jones,Zhang2005,Zhang2007}
---
> Hamiltonians can at least be \emph{simulated} are NMR qubits~\cite{Suter2006,Jones,Zhang2005}
241c241
< has been extended by various authors~\cite{Eisert2004,Kay,Landahl2005,Ericsson2005,Bose2005,Yung2006,Sun2006a,Sun2005c,Sun2005a,Lambropoulos2006,Lambropoulos2004,Kay2006,Kay2006a,Stolze2005,Jing-Fu2006,Ekert2004,Kostak2007},
---
> has been extended by various authors~\cite{Eisert2004,Kay,Landahl2005,Ericsson2005,Bose2005,Yung2006,Sun2006a,Sun2005c,Sun2005a,Lambropoulos2006,Lambropoulos2004,Kay2006,Kay2006a,Stolze2005,Jing-Fu2006,Ekert2004},
250d249
< The disadvantage of reliying on specific couplings strengths is that they the fidelity is typically not stable against disorder~\cite{Romito2,Mont,Chin}.
295,296c294
< to most other schemes. An experimental demonstration of this iterative approach
< has recently been given in a NMR system~\cite{Zhang2007}.%
---
> to most other schemes. %
316c314
< $|\mathbf{n}\rangle\equiv\sigma_{+}^{(n)}|\mathbf{0}\rangle$ with
---
> $|\mathbf{n}\rangle\equiv\sigma_{+}^{(k)}|\mathbf{0}\rangle$ with
320c318
< Finally we define the unnormalized states $|\phi_{k}\rangle$ recursively by $|\phi_{k+1}\rangle=PU_{k}|\phi_{k}\rangle$
---
> Finally we define the states $|\phi_{k}\rangle$ recursively by $|\phi_{k+1}\rangle=PU_{k}|\phi_{k}\rangle$
322,323c320
< The valve gates are two-qubit gates acting on qubits $N$ and $N+1$. Their ideal sequence is expressed in the canonical basis
< $\{|00\rangle,|01\rangle,|10\rangle,|11\rangle\}$ by 
---
> The ideal sequence of valve gates to be applied is then given by 
326c323
< V_{k}=(F_0^k)^{-1/2}\left(\begin{array}{cccc}
---
> V_{k}=\left({|\left\langle \mathbf{N}|\phi_{k-1}\right\rangle |}^{2}+{|\left\langle \mathbf{N}|\phi_{k}\right\rangle |}^{2}\right)^{-2}\left(\begin{array}{cccc}
328,331c325,330
< 0 & (F_0^{k-1})^{-1/2} & \left\langle \mathbf{N}|U_k|\phi_{k-1}\right\rangle ^{*}& 0 \\
< 0  & -\left\langle \mathbf{N}|U_k|\phi_{k-1}\right\rangle & (F_0^{k-1})^{-1/2} & 0\\
< 0  & 0 & 0 & 1\end{array}\right),\end{equation}
< where the minimal fidelity for quantum state transfer at the $k$th step
---
> 0 & \left\langle \mathbf{N}|\phi_{k-1}\right\rangle  & -\left\langle \mathbf{N}|\phi_{k}\right\rangle & 0 \\
> 0  & \left\langle \mathbf{N}|\phi_{k}\right\rangle ^{*} & \left\langle \mathbf{N}|\phi_{k-1}\right\rangle ^{*} & 0\\
> 0  & 0 & 0 & 1\end{array}\right).\end{equation}
> Ideally these gates act in a time-scale much shorter than the evolution
> of the chain, though this can be generalized~\cite{Bruder,Burgarth}.
> The minimal fidelity for quantum state transfer at the $k$th step
333c332
< F_{0}^{k}=1-\langle\phi_{k}|\phi_{k}\rangle.\end{equation}
---
> F_{0}^{k}=1-\langle\psi_{k}|\psi_{k}\rangle.\end{equation}
335,338c334
< Eq.~(\ref{eq:transfer}) in the presence of active gating. 
< Ideally the gates act in a time-scale much shorter than the evolution
< of the chain, though this can be generalized~\cite{Bruder,Burgarth}.
< For a given Hamiltonian one can easily compute the required
---
> Eq.~(\ref{eq:transfer}) in the presence of active gating. For a given Hamiltonian one can easily compute the required
362,367c358,360
< to the \emph{wrong} Hamiltonian. In principle, this could be a arbitrary time-dependent
< Hamiltonian. For simplicity we restrict ourselves to slowly varying Hamiltonians
< which are approximately constant during \emph{one} application of the protocol,
< but which have changed when the chain is used the next time. This assumption
< allows us to solve the problem for time-independent Hamiltonians and then average
< over different realizations.
---
> to the \emph{wrong} Hamiltonian. In principal, this could be a time-dependent
> Hamiltonian, but for simplicity we restrict ourselves to Hamiltonians
> that are approximately constant during one application of the protocol.
380,381c373,374
< applied to a \emph{perturbed} Hamiltonian where the $\delta_{n}$ are uniformly
< distributed in the interval $[-\Delta,\Delta],$ and the resulting minimal
---
> applied to a \emph{perturbed} Hamiltonian where the $\delta_{n}$ are randomly
> chosen in the interval $[-\Delta,\Delta],$ and the resulting minimal
393d385
<  We obtained similar results also for Gaussian distributed disorder and for on-site disorder.
410,412c402,403
< \caption{\label{fig:fidelity3}Fidelity that can be achieved using maximally $20$ steps
< of the valve protocol for a $XX$ chain of length $N=20$, i.e. $\mbox{max}_{k<20}F_{0}^{k}$. 
< Shown is the case where the ideal sequence is applied to \emph{unknown} disorder as a function of the error strength
---
> \caption{\label{fig:fidelity3}Achievable minimal fidelity, i.e. $\mbox{max}_{k}F_{0}^{k}$
> for a $XX$ chain of length $N=20$ as a function of the error strength
414c405
< give the fidelity $F_{0}$ of the original protocol~\cite{Bose2003} as a function of unknown disorder.
---
> give the minimal fidelity $F_{0}$ of the original protocol~\cite{Bose2003}.
422c413
< to known and \emph{unknown} disorder (such as slowly variying time-dependent disorder). This is a 
---
> to known and \emph{unknown} disorder (such as time-dependent disorder). This is a 
428c419
< \begin{acknowledgement}
---
> \section*{Acknowledgments}
436d426
< \end{acknowledgement}
522,524d511
< \bibitem{Romito2}
< A.~Romito, G.~de~Chiara, D.~Rossini and S.~Montangero,  Int. J. Quant. Inf., \textbf{4}, 519 (2006)
< 
558,559d544
< \bibitem{Zhang2007}
< J.~Zhang, N.~Rajendran, X~.Peng and D.~Suter, arXiv:0706.0352
668,669d652
< \bibitem{Kostak2007}
< V.~Kostak, G.~M.~Nikolopoulos and I. Jex, Phys. Rev. A \textbf{75}, 042319 (2007).
703,708d685
< \bibitem{Mont}
< G. De Chiara, D. Rossini, S. Montangero and R. Fazio, Phys. Rev. A \textbf{72}, 012323 (2005)
< 
< \bibitem{Chin}
< L. Dan and Z. Jing-Fu, Chin. Phys. \textbf{15}, 272 (2006) 
< 

